BiPart: A Parallel and Deterministic Multilevel Hypergraph Partitioner

Hypergraph partitioning is used in many problem domains including VLSI design, linear algebra, Boolean satisfiability, and data mining. Most versions of this problem are NP-complete or NP-hard, so practical hypergraph partitioners generate approximate partitioning solutions for all but the smallest inputs. One way to speed up hypergraph partitioners is to exploit parallelism. However, existing parallel hypergraph partitioners are not deterministic, which is considered unacceptable in domains like VLSI design where the same partitions must be produced every time a given hypergraph is partitioned. In this paper, we describe BiPart, the first deterministic, parallel hypergraph partitioner. Experimental results show that BiPart outperforms state-of-the-art hypergraph partitioners in runtime and partition quality while generating partitions deterministically.

==> abstract.tex <==
\begin{abstract}
    Hypergraph partitioning is a key step in many algorithms used in diverse domains including VLSI, linear algebra, Boolean satisfiability, and data-mining. Hypergraphs may contain many millions of nodes and edges, so it is important to have fast and scalable partitioners. In addition, some domains like VLSI design require \emph{deterministic} partitioners that produce exactly the same output every time they are used to partition a given hypergraph. Several serial and parallel hypergraph partitioners have been described in the literature but they do not guarantee deterministic results; in addition, some of them cannot handle large hypergraphs.
    
    This paper presents BiPart, a parallel balanced hypergraph partitioner that produces high-quality partitions competitive with state-of-the-art partitioners while guaranteeing determinism. BiPart has been designed so that if determinism is not important, execution can be speeded up by exploiting nondeterminism. Our experiments show that BiPart can successfully partition hypergraphs with tens of millions of nodes and hyperedges in a few seconds while guaranteeing determinism if needed.
\end{abstract}



==> coarse.tex <==
\subsection{Coarsening Algorithm}
Algorithm~\ref{euclid} describes the pseudocode for the coarsening algorithm used in BiPart. 
Coarsening in BiPart consists of two steps. In the  first step, BiPart performs a \textit{multi-node matching} and merges all the nodes in the same set into a single node in coarsened graph (Steps~\ref{alg1:matching}-\ref{alg1:endFor1}). In the second step, BiPart merges nodes in singleton sets with one of its neighbors that has been merged in the previous step (Steps~\ref{alg1:for2}-\ref{alg1:endFor2}).

Figure~\ref{fig:coarse} illustrates this with a hypergraph with nine nodes and three hyperedges. In the first step, BiPart performs multi-node matching. Figure~\ref{fig:coarse}(b) shows the result of this matching. The nodes in each of the disjoint sets in the matching are merged into a single node, as shown in Figure~\ref{fig:coarse}(c). Finally, sets with singleton nodes are merged with the larger merged nodes as shown in Figure~\ref{fig:coarse}(d).



==> comparison.tex <==
Table~\ref{tbl:perf} compares BiPart results with those obtained by running  Zoltan, KaHyPar and HYPE. 
BiPart is executed on 14 threads, and 
Zoltan  is executed on 14 processes, while KaHyPar, and HYPE are executed on a single thread since they are serial codes.



KaHyPar produces high-quality partitions but it took more than 1800 seconds to partition large graphs such as Random-10M, Random-15M, webbase, and Sat14. For the hypergraphs that KaHyPar can partition successfully, BiPart is always faster but worse in quality. HYPE runs on all inputs but the execution time and the quality of the partitions are always worse than BiPart.

Zoltan was able to partition all the hypergraphs in our test suite except for the largest hypergraph, Random-15M. 
 For the three largest hypergraphs Random-10M, NLPK and WB, BiPart is roughly 4X faster than Zoltan while producing partitions of comparable quality.
%sep
We also compared our results with other hypergraph partitioners, such as PaToH~\cite{patoh} and HMetis~\cite{hmetis}. We observed that the parallel execution time of BiPart is better than HMetis's and PaToH's serial time on large inputs. Since the source code for these partitioners is not available and due to the space constraints, we do not list those results here. We did not compare our results with Parkway since it frequently produces  segfaults.





==> kahyp.tex <==

%\addtolength{\tabcolsep}{-1pt}  
\begin{table*}
 %\scriptsize
 \small
 \begin{center}
 \caption{Performance of hypergraph partitioners (time is measured in seconds)}  \label{tbl:perf}
    \begin{tabular}{|r|r|r|r|r|r|r|r|r|r|}
        \hline
	    & \multicolumn{2}{c|}{BiPart (14)} & \multicolumn{2}{c|}{Zoltan (14)} & \multicolumn{2}{c|}{HYPE (1)}  & \multicolumn{2}{c|}{KaHyPar (1)}\\ \hline
	    \textbf{Inputs} & \textbf{Time} & \textbf{Edge cut} & \textbf{Time} & \textbf{Edge cut} &  \textbf{Time} & \textbf{Edge cut} & \textbf{Time} & \textbf{Edge cut} \\ \hline
	    \textbf{Random-15M} & \colorbox{green!20}{85.4} & \colorbox{green!20}{13,968,401} &  $-$ & $-$ & $>1,800$ & $15,628,206$ & > 1,800 & $-$ \\ \hline
	    \textbf{Random-10M} & \colorbox{green!20}{35.2} & \colorbox{green!20}{7,588,493} & 133.6 &  8,206,642  & $> 1,800$ & $8,816,800$ & > 1,800 & $-$ \\ \hline
	    \textbf{WB} & \colorbox{green!20}{7.9} & 13,853	& 31.4 & 35,212	& 42.2	& 819,661  & 581.5 & \colorbox{green!20}{11,457} \\ \hline
	    \textbf{NLPK} & \colorbox{green!20}{5.8}	& 98,010 & 	27.6	& 76,987 & 	58.8	& 651,396  & 784.3 & \colorbox{green!20}{59,205} \\ \hline
	    \textbf{Xyce} & \colorbox{green!20}{1.3}	& 1,134 & 4.1 &	1,190	& 11.8 &	549,364	&  412.4 & \colorbox{green!20}{420}	\\	\hline
      \textbf{Circuit1} & \colorbox{green!20}{0.7} & 3,439 & 4.2	& 2,314 & 10.9 &	371,700 & 524.1 & \colorbox{green!20}{2,171}	\\ \hline
	    \textbf{Webbase} & \colorbox{green!20}{0.3}	 &  \colorbox{green!20}{624} &	1.2 &	1,645 &	2.4 &455,492	 & > 1,800 & $-$ \\ \hline
       \textbf{Leon} & \colorbox{green!20}{0.9} &	112 & 5.4	& 81 &	3.8 &32460 &   354.6 & \colorbox{green!20}{59} \\ \hline
       \textbf{Sat14} & \colorbox{green!20}{7.6} & 15,394 & 44.3 & \colorbox{green!20}{5,748} & 61.3 & 524317 & > 1,800  &  $-$ \\ \hline
        \textbf{RM07R} & \colorbox{green!20}{0.8} &	22,350	& 3.9	& 56,296	& 19.1 & 151,570 &  880.0 & \colorbox{green!20}{17,532}	\\ \hline
        \textbf{IBM18} & \colorbox{green!20}{0.2} &	2,669	& 0.4	& 2,462 & 1.0	& 52,779 &453.9  & \colorbox{green!20}{1,915} \\ \hline
    \end{tabular}
 \end{center}
\end{table*}
%\addtolength{\tabcolsep}{1pt}  


==> kway-exp.tex <==
\subsection{Multiway Partitioning Performance}
\label{sec:exp-kway}

Figure~\ref{fig:kwayScale} shows the scaled execution time of BiPart for multiway partitioning of the two hypergraphs Xyce and WB. For both hypergraphs, the execution times are scaled by the time taken to create 2 partitions. If $k$ is the number of partitions to be created, the critical path through the computation increases as $O(log_2(k))$. The experimental results shown in Figure~\ref{fig:kwayScale} follow this trend roughly.

Tables~\ref{tbl:kway1} and \ref{tbl:kway2} show the performance of BiPart and the current state-of-the-art hypergraph partitioner, KaHyPar,
for multiway partitioning of a small graph IBM18 (Table~\ref{tbl:kway1}) and a large graph WB (Table~\ref{tbl:kway2}). We do not compare our results with Zoltan for $k$-way since their result is not deterministic. BiPart is much faster than KaHyPar; for example, KaHyPar times out after 30 minutes when creating 4 partitions of WB (9.8M nodes, 6.9M hyperedges), whereas BiPart can create 16 partitions of this hypergraph in just 20 seconds. However, when KaHyPar terminates in a reasonable time, it produces partitions with a better edge cut (for IBM18, the edge cut is on average 2.5X better).

We conclude that there is a tradeoff between BiPart and KaHyPar in terms of the total
running time and the edge cut quality. As shown in Tables~\ref{tbl:kway1} and \ref{tbl:kway2}, BiPart may be better suited than KaHyPar for creating a large number of partitions of large graphs while maintaining determinism.

